Investigating Automatic Scoring and Feedback using Large Language Models

Automatic grading and feedback have been long studied using traditional machine learning and deep learning techniques using language models. With the recent accessibility to high performing large language models (LLMs) like LLaMA-2, there is an opportunity to investigate the use of these LLMs for automatic grading and feedback generation. Despite the increase in performance, LLMs require significant computational resources for fine-tuning and additional specific adjustments to enhance their performance for such tasks. To address these issues, Parameter Efficient Fine-tuning (PEFT) methods, such as LoRA and QLoRA, have been adopted to decrease memory and computational requirements in model fine-tuning. This paper explores the efficacy of PEFT-based quantized models, employing classification or regression head, to fine-tune LLMs for automatically assigning continuous numerical grades to short answers and essays, as well as generating corresponding feedback. We conducted experiments on both proprietary and open-source datasets for our tasks. The results show that prediction of grade scores via finetuned LLMs are highly accurate, achieving less than 3% error in grade percentage on average. For providing graded feedback fine-tuned 4-bit quantized LLaMA-2 13B models outperform competitive base models and achieve high similarity with subject matter expert feedback in terms of high BLEU and ROUGE scores and qualitatively in terms of feedback. The findings from this study provide important insights into the impacts of the emerging capabilities of using quantization approaches to fine-tune LLMs for various downstream tasks, such as automatic short answer scoring and feedback generation at comparatively lower costs and latency.

==> notes.tex <==




% With the current availability of large language models, we are able to fine-tune the large language models for both automatic grading and feedback.  
% Fine-tuning pretrained language models (PLMs) has achieved significant performance improvements in natural language understanding tasks such as in automated grading for educational purposes. 
%talk about the imoortance of automatic grading to teachers 
%with this growing need for effective ways to ----, there is a need to develop and train better performing models especially high performing models 
Despite the increase in performance, LLMs require significant computational resources for fine-tuning and additional specific adjustments to enhance their performance for such tasks. To address these issues, Parameter Efficient Fine-tuning (PEFT) methods, such as LoRA and QLoRA, have been adopted to decrease memory and computational requirements in model fine-tuning. This work explores the effectiveness of PEFT-based quantized models for fine-tuning LLMs for automatic short answers (and essays) grading and feedback generation. 

We conducted experiments on an in-house essay grading and open-source datasets for our tasks. 


% across with the most recent reported performance for the SAF dataset in Table X. In Table Y, we report the results of the regression tasks and Table Z reports of the results of the comparison between the instruct-tuned and conventional fine-tuning with classification for the in-house dataset. We evaluated the models based on their Root Mean Square Error (RMSE) and Pearson's correlation coefficient ($p$), providing a dual perspective on both the accuracy and correlation strength of predictions relative to the true values. The ELMo model, as referenced from \cite{gaddipati2020comparative}, exhibited a RMSE of 0.978 and a $p$ value of 0.485, leading in terms of correlation among the models compared. In contrast, the GPT model demonstrated a higher RMSE of 1.082 and a significantly lower $p$ of 0.248, suggesting reduced prediction accuracy and correlation strength.

% Furthermore, the BERT and GPT-2 models, also benchmarked from Gaddipati et al.  \cite{gaddipati2020comparative}, showed similar trends with RMSE values of 1.057 and 1.065 and $p$ values of 0.318 and 0.274, respectively. These results indicate a consistent trend of higher RMSEs and lower correlation coefficients compared to the ELMo model. Interestingly, our 4-bit quantized LLama-2 models, both 7B and 13B, achieved identical RMSE values of 0.995 and $p$ values of 0.311. These outcomes demonstrate the effectiveness of the LLama-2 models in maintaining a balance between error minimization and correlation strength, despite the reduction in bit representation from the traditional 32-bit models. The comparable performance of the two LLama-2 variants also suggests a potential plateau in gains from increasing model complexity within the 4-bit quantized space.

% Keeping in the mind that these systems are developed to assist educators by reducing the time it takes to grade and generate custom feedback for each students based on specific questions. 

% In particular, NLP-based approaches have been used to predict grades a  

% Text-based answers such as short answers or essays, which are both considered as natural language answers with the main difference in the length, focus, and openness \cite{burrows2015eras}, are known to pose additional challenges for researchers over the years. 


% With teachers spending lesser time on manually grading and providing customized feedback, educators have more time to improve their educational practices and the students' experiences, such as creating and implementing more engaging learning activities.   



% In the context of automatic grading, machine learning (ML) and natural language processing (NLP) approaches have long been used to train models to made it partially or completely possible to automatically grade quizzes or exams \cite{suzen2020automatic}. 

% This has benefited teachers and instructors by reducing the time spent on grading and possible human error as well as in the cases where teachers or grading instructors are limited, such as in online learning. 

% To fine-tune LLMs for automatic grading tasks, where the goal is to provide a continuous value for the grade, regression analysis has been the most common approach to evaluating the results. However, LLMs are mainly pretrained and fine-tuned zero-shot and few-shot generative tasks, such as summarizations... \cite{}. These common applications have led to the evolution of prompt-based fine-tuning approaches, such as --,---, and --. 

% More recently, supervised instruction-tuning has shown improved performance with models like FLAN \cite{}. However, the instruct-based supervised fine-tuning is very limited to generative tasks and has been challenging to adapt to more discriminative tasks, like classification or regression, making it challenging to fine-tune for applications such as automated grading. 

% Recently, researchers have applied explored adapting instruction-tuning for classification purposes \cite{label lama} to predict the labels for task-specific applications with the recent release of \textit{LlamaForSequenceClassification }\cite{huggingface}. 

% These fine-tuning approaches shows exceptional promise in automated tasks like short answer and essay grading, highlighting the potential for further advancement in the field of education technology \cite{}.   

% P2 - However, these LLMs require significant computational resources for fine-tuning and additional specific adjustments to enhance their performance for discriminative tasks, such as predicting scores. 
% While these approaches have shown significant improvements, there is a need to explore newer approaches using large language models for automatic grading tasks.

% Instruction Fine-tuning is a special technique for tailoring LLMs to perform specific tasks based on explicit instructions. Unlike traditional fine-tuning, where a  model is trained on specific tasks, the instruction fine-tuning goes beyond by incorporating high-level instructions to guide the model's behavior. 

% QLoRA uses 4-bit quantization to compress a pretrained language model. The LM parameters are then frozen, and a relatively small number of trainable parameters are added to the model in the form of Low-Rank Adapters. During finetuning, QLoRA backpropagates gradients through the frozen 4-bit quantized pretrained language model into the Low-Rank Adapters. The LoRA layers are the only parameters being updated during training.

% \textbf{r}: This indicates the size of the reparameterization. Keep in mind that the smaller the value, the fewer parameters are trained. Training more parameters gives a better chance of learning the relationship between inputs and outputs, but it’s also more computationally expensive. A value of 16 is a reasonable compromise, allowing us to control parameters while still achieving a correct result.
% \textbf{lora\_alpha}: This factor adjusts the magnitude of the weight matrix. In smaller models, it usually doesn’t have a significant impact, but in larger models, it helps to give more weight to the fine-tuning in relation to the rest of the unchanged weights.
% target\_modules: This indicates which modules we want to train. It might seem like a challenging decision, primarily because you need to know the internal module names in the model. Fortunately, you can consult the documentation provided by Hugging Face, where it specifies the available modules for each model family.
% \textbf{lora\_dropout}: If you’ve trained deep learning models before, you are likely familiar with dropout. It’s used to prevent overfitting. In this case, considering the short training duration and limited data, you could experiment with a dropout value of 0.
% \textbf{bias}: There are three options — none, all, and lora\_only. For text classification, none is commonly used. For more complex tasks, you can choose between all and lora\_only.

